Adversarial Attacks on Black Box Video Classifiers: Leveraging the Power of Geometric Transformations

When compared to the image classification models, black-box adversarial attacks against video classification models have been largely understudied. This could be possible because, with video, the temporal dimension poses significant additional challenges in gradient estimation. Query-efficient black-box attacks rely on effectively estimated gradients towards maximizing the probability of misclassifying the target video. In this work, we demonstrate that such effective gradients can be searched for by parameterizing the temporal structure of the search space with geometric transformations. Specifically, we design a novel iterative algorithm Geometric TRAnsformed Perturbations (GEO-TRAP), for attacking video classification models. GEO-TRAP employs standard geometric transformation operations to reduce the search space for effective gradients into searching for a small group of parameters that define these operations. This group of parameters describes the geometric progression of gradients, resulting in a reduced and structured search space. Our algorithm inherently leads to successful perturbations with surprisingly few queries. For example, adversarial examples generated from GEO-TRAP have better attack success rates with ~73.55% fewer queries compared to the state-of-the-art method for video adversarial attacks on the widely used Jester dataset. Overall, our algorithm exposes vulnerabilities of diverse video classification models and achieves new state-of-the-art results under black-box settings on two large datasets. Code is available here: https://github.com/sli057/Geo-TRAP

==> images/loss_curves.tex <==
\begin{figure}[htbp]
	\centering
	\subfloat[]{
		\label{fig:loss_curves}
		\includegraphics[width=0.48\columnwidth]{NeuIPS/images/loss_curves_targeted_12.pdf} } 
	\hfill
	\subfloat[]{
		\label{fig:gradient_curves}
		\includegraphics[width=0.48\textwidth]{NeuIPS/images/gradient_curves_targeted_12.pdf} } 
	\caption{Following \cite{jiang2019black}, we evaluate the gradient estimation quality by calculating the cosine similarity between the ground truth gradient $\bm{g}*$ and the estimated gradient $\bm{g}$ calculated by different attack methods. The results (numbers shown in the table * 1e-3) are based on attacks on 1000 randomly chosen videos and the cosine similarity values in the first attack iteration are averaged. We choose the first iteration because the initial $\bm{g}*$  is same for different attack methods. Evaluation results with different datasets and loss functions can be found in the supplementary material. } %All the curves yield $\text{AUC} \geq 0.9$. }
	\label{fig:expain} 
\end{figure}


==> slides/presentation.tex <==
\begin{frame}
\frametitle{~}
\centering
\textcolor{ucr_blue}{\bf\Huge{Introduction}}
\end{frame}


\begin{frame}[t]{\bf Black-box Adversarial Attack on Video Classifiers}

\begin{itemize}\justifying
    \item \textbf{Problem Statement:} How to create imperceptible video perturbation, so that the perturbed video is misclassified by the black-box model?
\end{itemize}
\pause
\begin{figure}
    \centering
    \includegraphics<2>[width=0.9\textwidth]{slides/slides_images/problem.png}
\end{figure}

\end{frame}


\begin{frame}[t]{\bf Black-box Adversarial Attack on Video Classifiers}

\begin{itemize}\justifying
    \item \textbf{Effective attacks:} Better gradient estimation is the key to query-based black-box attack.
\end{itemize}
\pause
\begin{figure}
    \begin{subfigure}{0.4\textwidth}
    \centering
    % include first image
    \includegraphics<2>[width=\textwidth]{slides/slides_images/white_box.png} 
    \caption{Illustration of White-box attack}
    \end{subfigure}
    \hfil
    \begin{subfigure}{0.4\textwidth}
    \centering
    % include second image
    \includegraphics<2>[width=\textwidth]{slides/slides_images/black_box.png}
    \caption{Illustration of Black-box attack}
    \end{subfigure}
\end{figure}

\end{frame}


\begin{frame}
\frametitle{~}
\centering
\textcolor{ucr_blue}{\bf\Huge{Gradient Estimation}}
\end{frame}


\begin{frame}{\bf Gradient Estimation: Sampling Directions}
    \begin{columns}
    %
    \begin{column}{.45\textwidth}
      \minipage[c][0.65\textheight][s]{\columnwidth}
      \vspace{0.05\textheight}

    \begin{itemize}\justifying
    \setlength\itemsep{2em}
        \item A simplified algorithm.
        \item<2> How to sample  $\bm{\pi}$ is important!
    \end{itemize}

      \endminipage
    \end{column}
    %
    \begin{column}{.55\textwidth}

      % for top aligned images use minipage
        \minipage[c][0.8\textheight][s]{\columnwidth}    
           \begin{figure}
            \centering
            \includegraphics[width=\textwidth]{%
              slides_images/simplified_grad_est.png} 
            \caption{Gradient estimation for high dimensional function}
            \addtocounter{figure}{-1}
        \end{figure}

        \endminipage
    \end{column}
  \end{columns}
\end{frame}


\begin{frame}{\bf Gradient Estimation: Query-efficiency}
    \begin{columns}
    %
    \begin{column}{.45\textwidth}
      \minipage[c][0.65\textheight][s]{\columnwidth}
      % \vspace{0.05\textheight}

    \begin{itemize}\justifying
    \setlength\itemsep{1em}
        \item $\bm{\pi}$ is in high dimensional space $D=T\times H\times W\times C$, where $T$ is the number of frames, $H$ and $W$ are the height and width of the frames, $C$ is the number of channels. 

        \item<2,3> Higher dimensionality leads to more number of queries $\rightarrow$ becomes worse compared to query-based image attacks.
        
        \item<3> \textbf{Goal:} Query-efficient query-based video attack!

    \end{itemize}

      \endminipage
    \end{column}
    %
    \begin{column}{.55\textwidth}

      % for top aligned images use minipage
        \minipage[c][0.8\textheight][s]{\columnwidth}    
           \begin{figure}
            \centering
            \includegraphics[width=\textwidth]{%
              slides_images/simplified_grad_est.png} 
            \caption{Gradient estimation for high dimensional function}
            \addtocounter{figure}{-1}
        \end{figure}

        \endminipage
    \end{column}
  \end{columns}
\end{frame}


\begin{frame}
\frametitle{~}
\centering
\textcolor{ucr_blue}{\bf\Huge{Motivation of Proposed Work}}
\end{frame}


\begin{frame}{\bf Motivation: Reduce the Search Space }
    \begin{columns}
    %
    \begin{column}{.45\textwidth}
      \minipage[c][0.65\textheight][s]{\columnwidth}
      % \vspace{0.05\textheight}

    \begin{itemize}\justifying
    \setlength\itemsep{2em}
        \item To estimate better gradient $\bm{g}$.
        \item<2,3> Sample $\bm{\pi}$ in a subspace (dimensionality reduction), which contains more effective $\bm{\pi}$.
        \item<3> Consider the intrinsic different between images and videos, i.e., the temporal dimension and aim to disrupt the motion context of videos.
    \end{itemize}

      \endminipage
    \end{column}
    %
    \begin{column}{.55\textwidth}

      % for top aligned images use minipage
        \minipage[c][0.8\textheight][s]{\columnwidth}    
           \begin{figure}
            \centering
            \includegraphics[width=\textwidth]{%
              slides_images/simplified_grad_est.png} 
            \caption{Gradient estimation for high dimensional function}
            \addtocounter{figure}{-1}
        \end{figure}

        \endminipage
    \end{column}
  \end{columns}
\end{frame}


\begin{frame}
\frametitle{~}
\centering
\textcolor{ucr_blue}{\bf\Huge{Proposed Method:\\[0.5em] GEOmetrically TRAnsformed Perturbations (GEO-TRAP)}}
\end{frame}


\begin{frame}{\bf Proposed Method: GEO-TRAP}
    \begin{columns}
    %
    \begin{column}{.45\textwidth}
      \minipage[c][0.65\textheight][s]{\columnwidth}
      % \vspace{0.05\textheight}

    \begin{itemize}\justifying
    \setlength\itemsep{2em}
        \item Randomly sample $\bm{r_{\text{frame}}} \in \mathbb{R}^{H\times W\times C}$, then warp $\bm{r_{\text{frame}}}$ with $T$ random geometric transformations to get $\bm{\pi} \in \mathbb{R}^{T\times H\times W\times C}$

    \end{itemize}

      \endminipage
    \end{column}
    %
    \begin{column}{.55\textwidth}

      % for top aligned images use minipage
        \minipage[c][0.8\textheight][s]{\columnwidth}    
           \begin{figure}
            \centering
            \includegraphics[width=\textwidth]{%
              slides_images/simplified_grad_est.png} 
            \caption{Gradient estimation for high dimensional function}
            \addtocounter{figure}{-1}
        \end{figure}

        \endminipage
    \end{column}
  \end{columns}
\end{frame}


\begin{frame}[t]{\bf Proposed Method: GEO-TRAP}

\begin{itemize}\justifying
    \item \textbf{Dummy Illustration:} Warping random noise $r_{\text{frame}}$ to create search directions for gradients
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{slides/slides_images/r_frame.png}
\end{figure}

\end{frame}


\begin{frame}[t]{\bf Proposed Method: GEO-TRAP}

\begin{itemize}\justifying
    \item Randomly sample $\bm{r_{\text{frame}}} \in \mathbb{R}^{H\times W\times C}$, then warp $\bm{r_{\text{frame}}}$ with $T$ random geometric transformations to get $\bm{\pi} \in \mathbb{R}^{T\times H\times W\times C}$.
\end{itemize}
\vfill
\textbf{Why does it work?}

\begin{itemize}\justifying
\setlength\itemsep{1em}
    \item Temporally structured perturbations. 
    \begin{itemize}\justifying
        \item[$\bullet$] Geometric progression in the temporal dimension.
    \end{itemize}
    
    \item Assume the degrees of freedom of the geometric transformation is $F$, the dimensionality $D$ is then reduced from $(T\times H\times W\times C$) to $(H\times W\times C)+ (T\times F)$ where, $F << T\times H\times W\times C$.
    \begin{itemize}\justifying
        \item[$\bullet$] e.g. $F=6$  for affine transformation.
    \end{itemize}

\end{itemize}

\end{frame}



\begin{frame}[t]{\bf Why GEO-TRAP works?}

\begin{columns}
    %
    \begin{column}{.45\textwidth}
      \minipage[c][0.65\textheight][s]{\columnwidth}
      % \vspace{0.05\textheight}

    \begin{itemize}\justifying
    \setlength\itemsep{1em}
        \item Cosine similarity between the estimated $\bm{g}$ and the ground truth $\bm{g}^\star$, averaged over 1000 randomly chosen samples.
        
        \item \textbf{Takeaway:} $\geotrap$ estimates better gradients compared to baselines.

    \end{itemize}

      \endminipage
    \end{column}
    %
    \begin{column}{.55\textwidth}

      % for top aligned images use minipage
        \minipage[c][0.8\textheight][s]{\columnwidth}    
           \begin{figure}
            \centering
            \includegraphics[width=0.9\textwidth]{images/sec_5_inner_prod.pdf}
            \caption{Measure the quality of estimated $\bm{g}$}
        \end{figure}

        \endminipage
    \end{column}
  \end{columns}

\end{frame}


\begin{frame}[t]{\bf Why GEO-TRAP works?}

\begin{itemize}\justifying
    \item \textbf{Better gradients} leads to quicker convergence, thus \textbf{fewer number of queries} required.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/sec_5_loss.pdf}
\end{figure}

\end{frame}


\begin{frame}[t]{\bf Experimental Result}\justifying

\textbf{Evaluation Metric:}
\begin{itemize}\justifying
    \item \textbf{Success Rates (SR):} total success rate of attack within query and perturbation budgets.
    \item \textbf{Average Number of Queries (ANQ):} the average  total queries from attacks for all videos (including failed ones).
\end{itemize}
\vfill
\pause
\textbf{Datasets:}
\begin{itemize}\justifying
    \item \textbf{UCF-101} \supercite{soomro2012ucf101}: UCF-101 includes 13320 videos from 101 human action categories (e.g., applying lipstick, biking). 
    \item \textbf{20BN-JESTER (Jester)} \supercite{materzynska2019jester}: Jester includes 27 kinds of gesture videos recorded by crowd-sourced workers (e.g., sliding hand left, sliding two fingers right).
\end{itemize}

\end{frame}


\begin{frame}[t]{\bf Experimental Result}

\begin{itemize}\justifying
    \item \textbf{Takeaway:} \geotrap achieves the same or higher attack Success Rates (SR) compared to other methods, and requires fewer Average Number of Queries (ANQ).
    \item More results and analysis in the paper.
\end{itemize}

\input{table}

\end{frame}


\begin{frame}{\bf Conclusion}

\begin{itemize}\justifying
\setlength\itemsep{1em}
    \item We propose a new black-box video attack method, which
    parameterizes the video search space into an image search space and a geometric transformation parameter search space.
    
    \item With the reduced and temporally structured search space, we are able to achieve higher attack success rate with fewer queries.
\end{itemize}

\end{frame}

==> slides/table.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table}[b]
\centering
\caption{\geotrap demonstrates highly successful untargeted attacks with fewer queries.}

\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{c|c|cc|cc|cc|cc}
\hline
\rowcolor{black!10}
 &  & \multicolumn{8}{c}{\textbf{Black-box Video Classifiers}}                                                 \\
 \cline{3-10}
\rowcolor{black!10}
 &  & \multicolumn{2}{c|}{\textbf{C3D}}  & \multicolumn{2}{c|}{\textbf{SlowFast}}                                           & \multicolumn{2}{c|}{\textbf{TPN}}                                                 & \multicolumn{2}{c}{\textbf{I3D}}                                                 \\
 \cline{3-10}
\rowcolor{black!10} \multirow{-3}{*}{\textbf{Datasets}}
                         &       \multirow{-3}{*}{\textbf{Methods}}           & ANQ ($\downarrow$)                     & SR ($\uparrow$)                                 & ANQ ($\downarrow$)                             & SR ($\uparrow$)                                 & ANQ ($\downarrow$)                               & SR ($\uparrow$)                                  & ANQ ($\downarrow$)                              & SR ($\uparrow$)                                  \\ \hline
\multirow{3}{*}{Jester}  & \textsc{HeuristicAttack}~\supercite{wei2020heuristic}        & 4699                     & 99.0\%                              & 3572                             & 98.1\%                              & 4679                              & 82.0\%                              & 4248                              & 98.1\%                              \\ \cline{2-10} 
                         & \textsc{Motion-Sampler Attack}~\supercite{zhang2020motion}    & 4549                     & 99.0\%                              & 1906                             & 100\%                              & 6269                              & 91.3\%                              & 3029                              & 99.4\%                              \\ \cline{2-10} 
                         & \geotrap (\textbf{Ours})                    & \textbf{1602}            & \textbf{100\%}                     & \textbf{521}                     & \textbf{100\%}                      & \textbf{3315}                     & \textbf{92.4\%}                     & \textbf{1599}                     & \textbf{100\%}                      \\ \hline
\multirow{3}{*}{UCF-101}     & \textsc{HeuristicAttack}       & \textbf{5206} & 70.2\%          & 3507         & 87.2\%          & \textbf{6539}         &  71.8\%          &  6949          &  84.7\%          \\ \cline{2-10} 
                         & \textsc{Motion-Sampler Attack}    & 14336                     &  81.6\%          &  4673         &  97.2\%          &  20369          &  75.8\%          &  7400          &  94.4\%          \\ \cline{2-10} 
                         & \geotrap (\textbf{Ours})                    & {11490}            &  \textbf{86.2\%} &  \textbf{1547} &  \textbf{98.8\%} &  {17716} &  \textbf{76.1\%} &  \textbf{4887} &  \textbf{97.4\%} \\ \hline
\end{tabular}
}
\end{table}

==> tables/cosine_sim_bar_plot.tex <==
% ============================
\def\axisdefaultwidth{240pt}
\pgfplotsset{
  every axis/.append style = {thick},tick style = {thick,black},
  %
  % #1 = x, y, or z
  % #2 = the shift value
  /tikz/normal shift/.code 2 args = {%
    \pgftransformshift{%
        \pgfpointscale{#2}{\pgfplotspointouternormalvectorofticklabelaxis{#1}}%
    }%
  },%
  %
  range3frame/.style = {
    tick align        = outside,
    scaled ticks      = false,
    enlargelimits     = false,
    ticklabel shift   = {10pt},
    axis lines*       = left,
    line cap          = round,
    clip              = false,
    xtick style       = {normal shift={x}{10pt}},
    ytick style       = {normal shift={y}{10pt}},
    ztick style       = {normal shift={z}{10pt}},
    x axis line style = {normal shift={x}{10pt}},
    y axis line style = {normal shift={y}{10pt}},
    z axis line style = {normal shift={z}{10pt}},
  }
}

\pgfplotsset{every axis legend/.append style={    
    at={(0.05,1.0)},
    anchor=north west,
    font = \scriptsize,
    legend columns=-1,
    /tikz/every even column/.append style={column sep=0.15cm}
        }}
\begin{tikzpicture}[scale=0.75, transform shape]
\begin{axis}[
%legend columns=-1,
legend cell align=left,
every axis plot post/.style={/pgf/number format/fixed},
ybar=2pt,
bar width=10pt,
ymin=0,
axis on top,
ymax=2.5,
xtick=data,
xticklabels={\geotrap, \cite{zhang2020motion}, \textsc{One-Noise}, \textsc{Multi-Noise}},
point meta=explicit symbolic,
nodes near coords align={vertical},
axis lines = left,
%xlabel=Cores,
ylabel=$\langle\rangle$,
enlarge x limits=0.2,
%enlarge y limits={abs=0.5},
symbolic x coords={ours, MS, ON, MN},
%restrict y to domain*=0:11, % Cut values off at 14
visualization depends on=rawy\as\rawy, % Save the unclipped values
after end axis/.code={ % Draw line indicating break
\draw [ultra thick, white] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
    },
nodes near coords={\scriptsize{\pgfmathprintnumber{\rawy}}},
every node near coord/.append style={
                        anchor=west,
                        rotate=90
                },
axis lines*=left,
clip=false,
area legend
]
\addplot[fill=darkpastelgreen!40, rounded corners=1pt] coordinates {(ours, 2) (ON, 0.83) (MS, 1.42) (MN, 0.98)};
\addplot[fill=yellow!40] coordinates {(ours, 1.49) (ON, 1.06) (MS, 1.19) (MN, 0.99)};
\legend{Targeted Attack, Untargeted Attack};
\end{axis}
\end{tikzpicture}

==> tables/cosine_similarity.tex <==
\begin{table}[htb]
\centering
\caption{Following \cite{jiang2019black}, we evaluate the gradient estimation quality by calculating the cosine similarity between the ground truth gradient $\bm{g}*$ and the estimated gradient $\bm{g}$ calculated by different attack methods. The results (numbers shown in the table * 1e-3) are based on attacks on 1000 randomly chosen videos and the cosine similarity values in the first attack iteration are averaged. We choose the first iteration because the initial $\bm{g}*$  is same for different attack methods. Evaluation results with different datasets and loss functions can be found in the supplementary material. }
\label{tab:cosine_similarity_supp}
%\small
%\resizebox{\columnwidth}{!}{
\input{NeuIPS/tables/cosine_sim_bar_plot}

%}
\end{table}
